A Formally Verified Lightning Network

In this work we use formal verification to prove that the Lightning Network (LN), the most prominent scaling technique for Bitcoin, always safeguards the funds of honest users. We provide a custom implementation of (a simplification of) LN, express the desired security goals and, for the first time, we provide a machine checkable proof that they are upheld under every scenario, all in an integrated fashion. We build our system using the Why3 platform.

==> src/experiment.tex <==
\section{Experiment}
\TODO{reread this section, move important parts to earlier sections, and remove}
We have designed our formal verification effort in the form of a security
experiment. This experiment consists of a \emph{system state}
%together with strict constraints on its validity
and a range of possible \emph{adversarial
      messages}, each transforming the system state accordingly. The adversary can
send any series of messages, as long as they respect a few basic constraints.
This is equivalent to simply ignoring invalid messages. The experiment is said to be
successful if every valid adversarial message transforms the system state into a
new state that is also valid.

We formally prove that, given an explicitly defined initial system state and a
series of valid adversarial actions, the resulting state is also valid.

In the following we explain modelling of the party, the system state, the
adversary and its messages in
more detail. We also provide detailed intuition on the semantics of valid
system states and adversarial messages.


\paragraph{Modelling of the party.}
To model the user of the system we use environment - orders sended by environment to the party correspond to action chosen by a user of the system. Below we provide exhaustive list of such actions, together with description of a scenarios they intend to model.

\begin{enumerate}
      \item \texttt{PayOnChain amount}: This order an on-chain payment of
            \texttt{amount} coins from the honest party to the counterparty. If not enough funds
            are available, the order is ignored. The order is also ignored if channel is not opened yet and party is not in Standby state.
      \item \texttt{EnvOpenChannel amount}: This order to initiate
            the opening of an off-chain channel, with itself as funder and initial owner of
            \texttt{amount} coins, by sending an \texttt{OpenChannel amount} message to the
            counterparty. If not enough founds are available, the order is ignored.
      \item \texttt{PayOffChain amount}: This order the honest party to initiate an
            off-chain payment of \texttt{amount} coins to its counterparty over the already
            established channel by sending an \texttt{Initializer} message to the
            counterparty.
      \item \texttt{CloseNow}: This order the honest party to exit a channel (is such exists).
      \item \texttt{JustCheckGamma}: This no-operation order. It's goal is to wake up honest party, such that it could perform periodic check of gamma state.
\end{enumerate}

Upon delivery of one these messages execution of party code began. Party could see current state of $\Gamma$ and could interact with signature functionality (immediately getting response). When execution of party stops, it generates a list of messages he sent to $\Gamma$ and counterparty. Such messages are to delivered immediately, but put in queue.

\texttt{deltaWake} is the maximum number of rounds between two activations of
the honest party: \texttt{work} needs this maximum to be enforced by the
experiment in order to uphold security.

The intuitive description provided above is formalized by construction of the experiment. Experiment will keep track of some expectations over party behavior (for example it will track how money the party should have). Given a adversary chosen message from environment, experiment will modify the expectations accordingly - for example given outgoing \texttt{PayOnChain amount} order, it will decrement expected amount of money that party should have. The detailed description of experiment is provided below.


\paragraph{System state.}
% The channel and ledger data are stored in the combined \texttt{gamma} structure.

Ledger and channel transformations take place according to distinct ledger and
channel protocols. Given a pair of such protocols, the success or failure of the
experiment determines whether the protocols \emph{realize} the desired system
\emph{functionality}, with the latter being defined by the system state
constraints. \TODO{maybe we shouldn't say that our definition is a realization of any functionality, we could present it as 'no lose money property' of the system}


\paragraph{Adversarial messages and system transformations.}
The adversary \adversary is any (unbounded) machine. It controls the moves of
the corrupted party. I also have some control over networking queue and orchestrates the execution by providing inputs of the paries (by proving environment orders).
%The adversarial messages drive transformations of the system state via the \texttt{step} function.
The experiment consists of a series of steps, with each transforming the
\emph{system state} according to a single \emph{adversarial action} \TODO{change term to choice, as ee have planty of messages, and the term  'message' is heavly overloaded already}. This action are the moves of the \adversary in the security game. The following actions are available to adversary:

\paragraph{Adversarial message constraints.}
Each adversarial message must respect a set of constraints. In our
implementation, invalid messages are either unrepresentable (as messages must be
elements of the \texttt{adversaryMoveT} type), or filtered out by the
\texttt{moveApplicable} predicate. This is equivalent to allowing arbitrary
messages, but simply ignoring invalid ones. The following constraints have to be
obeyed:
\begin{enumerate}
      \item For \texttt{IncrementTime} messages, the honest party must not exceed the
            maximum inactive number of rounds (\texttt{deltaWake}),
      \item A environment order \texttt{exit} that instructs a party to close its channel cannot be sent
            unless the ledger sees the channel as already open,
      \item An off-chain payment instruction (i) cannot be sent unless both the
            ledger and the party see the channel as already opened and (ii) cannot require
            paying more than the available off-chain balance,
      \item An on-chain payment instruction (i) cannot require paying more than
            the available on-chain balance and (ii) cannot be dispatched while another
            on-chain payment is pending \TODO{check if the last is still needed.}
            \TODO{There are two commented-out requirements: one is that the channel is
                  Normal and the other mentions an old version of \texttt{reactToDispute}. Are
                  these still relevant?}
      \item A message that delivers a pending message to the ledger must specify a
            message that is indeed in the queue. \TODO{this is very low level, maybe not need to mention it.}
      \item Adversary cannot increase time if doing would invalidate time bound on delivery of message form queue, or time bound on party inactivity.
\end{enumerate}

\paragraph{Experiment goal.}
In the experiment, adversary wins if he violated following property:

If time $\Delta$ passed from the first moment when environment order (valid)
\texttt{exit}, then party have more funds on chain than initial amount reduced by sum of payments order by environment.

Finally, we could define no-lsoe-money property:

Party implementation

\section{Protocol}
\subsection{Ledger handler}
Our implementation of the ledger handler \texttt{gammaProcesMsg} handler is
designed to accept messages that have been dequeued from the ledger message
queue and are accompanied by the time of submission. All such messages contain a
suitable transaction and a valid signature on it by the message sender, except
when otherwise specified. \texttt{deltaNet} is the maximum number of rounds that
a message for the ledger can stay unprocessed: \texttt{gammaProcesMsg} only
upholds security if this maximum is enforced by the experiment. The following
kinds of ledger messages are allowed:
\begin{enumerate}
      \item \texttt{MoveOwnCoinsOnChain args}: When \texttt{args.destination} is
            \texttt{OtherParty}, a simple on-chain payment of \texttt{args.amount} coins
            from the honest party to the counterparty is carried out if the former has
            enough coins on-chain. When \texttt{args.destination} is \texttt{Channel} and
            the channel is closed, the channel is established. This corresponds to the
            on-chain finalization of the LN funding transaction.
      \item \texttt{OpenDispute halfSigned}: When the channel is open and the
            transaction of type \texttt{halfSigned} is signed by both channel parties, the
            channel enters the \texttt{DisputeOpen} state. This corresponds to the on-chain
            finalization of the LN commitment transaction.
      \item \texttt{ClaimAfterTimeout}: When the channel is in the
            \texttt{DisputeOpen} state and given that the dispute period has elapsed, this
            message prompts the channel to close and the rightful balances to be returned to
            the parties on-chain. This message is not accompanied by a transaction or
            signature. In LN, it corresponds to the party that had published a commitment
            transaction waiting for the dispute timelock to expire and gaining access to its
            coins. This is the case in which no revocation transaction was published and
            thus no punishment took place --- both parties acted honestly.
      \item \texttt{Revoke}: When the channel is in the \texttt{DisputeOpen} state and
            the corresponding commitment transaction is accompanied by a revocation
            signature by the counterparty of the current message sender, this message
            prompts the channel to close and all channel funds to be given on-chain to the
            current message sender, thus punishing its counterparty. In LN, it corresponds
            to a publication of a revocation transaction. This is the case in which the
            counterparty had maliciously published earlier a commitment transaction that has
            already been revoked and thus corresponds to a past, invalid channel state.
            \TODO{rename Revoke to Punish in code where appropriate}
\end{enumerate}

\subsection{Channel party protocol}
Our implementation of the channel party protocol \texttt{work} is
designed to accept both messages by the environment and by the counterparty.
On its every activation, if the honest party is the channel
funder and it has submitted the funding tx, it checks whether the ledger has
included it on every activation and informs its counterparty with a
\texttt{ChannelReadyByFunder} message when so. Additionally, if the channel is
open, it always checks the ledger for outdated commitment transactions and
publishes the corresponding revocation transaction if one is found. More
specific actions are determined by the specific message. The following
\texttt{FromEnv} messages are defined:
\begin{enumerate}
      \item \texttt{PayOnChain amount}: This prompts an on-chain payment of
            \texttt{amount} coins from the honest party to the counterparty. If enough funds
            are available, the corresponding transaction is signed and added to the ledger
            queue.
      \item \texttt{EnvOpenChannel amount}: This prompts the honest party to initiate
            the opening of an off-chain channel, with itself as funder and initial owner of
            \texttt{amount} coins, by sending an \texttt{OpenChannel amount} message to the
            counterparty.
      \item \texttt{PayOffChain amount}: This prompts the honest party to initiate an
            off-chain payment of \texttt{amount} coins to its counterparty over the already
            established channel by sending an \texttt{Initializer} message to the
            counterparty.
      \item \texttt{CloseNow}: This prompts the honest party to publish the latest
            commitment transaction in order to close the already established channel.
      \item \texttt{JustCheckGamma}: This message has no specific goal other than
            prompting the honest party to carry out the two standard checks discussed above.
\end{enumerate}
The following \texttt{FromParty} messages are associated with channel opening:
\begin{enumerate}
      \item \texttt{OpenChannel amount}: This prompts the receiver to become a fundee
            to a new channel. It responds with \texttt{AccpetChannel amount} to its
            counterparty.
      \item \texttt{AcceptChannel amount}: This prompts the funder to create and
            sign its first commitment transaction, as well as create the funding
            transaction, which are sent to the counterparty with a \texttt{FundingCreated}
            message.
      \item \texttt{FundingCreated fundingTx fundeesHalfSignedCommitmentData}:
            \TODO{either rename Split to CommitmentData in code, or the reverse here} This
            prompts the fundee to create and sign its first commitment transaction, which
            is sent to the counterparty with a \texttt{CommitmentSigned} message.
      \item \texttt{CommitmentSigned fundersHalfSignedCommitmentData}: \TODO{same name
                  change} This prompts the funder to sign the funding transaction and add it
            to the ledger queue. As discussed above, when the funding transaction is
            finalized, the funder sends \texttt{ChannelReadyByFunder} to the fundee.
      \item \texttt{ChannelReadyByFunder}: This prompts the fundee to consider the
            channel opened and send \texttt{ChannelReadyByFundee} to the funder.
      \item \texttt{ChannelReadyByFundee}: Finally, this prompts the funder to
            consider the channel opened.
\end{enumerate}
The following \texttt{FromParty} messages are associated with payment in the
channel:
\begin{enumerate}
      \item \texttt{Initializer}: This prompts the payee to create and sign a new
            commitment transaction which reflects the new channel balance. This is sent to
            the counterparty with a \texttt{Commit} message.
      \item \texttt{Commit}: This prompts the payer to create and sign the
            corresponding commitment transaction, as well as revoke its previously valid
            commitment transaction. This data is communicated to the counterparty with a
            \texttt{CommitAndRevokeAndAck} message.
      \item \texttt{CommitAndRevokeAndAck}: This prompts the payee to revoke its
            previously valid commitment transaction. The revocation is sent to the payer
            with a \texttt{RevokeAndAck} message. This completes the payment for the payee.
      \item \texttt{RevokeAndAck}: This informs the payer that the payment is
            complete.
            \TODO{describe expectedAmount and cancel if needed}
\end{enumerate}
\texttt{deltaWake} is the maximum number of rounds between two activations of
the honest party: \texttt{work} needs this maximum to be enforced by the
experiment in order to uphold security.

\subsection{Invariant of the experiment}
\paragraph{System state constraints.}
A system state during experiment obeys the following set of invariants:
\begin{enumerate}
      \item The honest party has been activated at most \texttt{deltaWake} rounds ago,
      \item Messages to the ledger do not stay unprocessed for more than
            \texttt{deltaNet} rounds,
      \item Party balances are non-negative during and after opening,
      \item Signatures stored by the signature functionality and the honest party
            coincide, \TODO{discuss removal}
      \item The most recent commitment transaction held by the honest party (if any)
            is signed by the counterparty,
      \item All revocation transactions held by the honest party are signed by the
            counterparty,
      \item The honest party's coins are non-negative and equal those displayed to the
            user plus those locked for funding a channel under creation, \TODO{discuss
                  removal}
      \item The honest party never signs a revoked commitment transaction,
      \item The channel is funded with positive coins on the funder's side and with no
            coins on the fundee's side,
      \item The honest party correctly keeps track of the number of payments that have
            taken place off-chain and of transactions that it has published on-chain,
      \item \TODO{signedSplitsSpec have not been mentioned, should they?},
      \item In case the channel is open, the balances stored by the honest party
            correspond to those in both latest commitment transactions,
      \item Both on- and off-chain balance modifications are tracked correctly by the
            honest party.
\end{enumerate}


==> src/signatures.tex <==
\section{Digital Signatures}
\label{sec:signatures}
\TODO{split between intro and model}
Digital Signatures~\cite{lamport1979constructing} are one of the most
fundamental and widely used cryptographic primitives. It is heavily used in
many applications, including Bitcoin. The standard \emph{primitive} (i.e.,
interface) provides three algorithms:
\begin{itemize}
  \item $(\pk{}, \sk{}) \overset{\$}\gets \mathsf{KeyGen}(1^\lambda)$: a
  probabilistic algorithm that takes as input a security parameter and outputs
  a verification (public) \& signing (private) key pair.
  \item $\sigma \overset{\$}\gets \mathsf{Sign}(\sk{}, m)$: a probabilistic
  algorithm that takes as input the signing key and a message string and
  outputs a \emph{signature} for this message.
  \item $\{0, 1\} \gets \mathsf{Verify}(\pk{}, m, \sigma)$: a deterministic
  algorithm that takes a verification key, a message and a signature and
  outputs whether the verification succeeded or not.
\end{itemize}
Informally, signatures created with \textsf{Sign}() should always
\textsf{Verify}() (correctness) and parties without knowledge of the signing
key should be unable to forge signatures (unforgeability). Concrete
implementations of the three algorithms that uphold these two guarantees are
called \emph{constructions}.

From a cryptographic perspective, the security of any digital signatures
construction is only \emph{computational}, i.e., it can be broken by a
sufficiently powerful adversary. In the simplest case, an adversary with no
computational limits (i.e., \emph{unbounded}) can forge a signature by
brute-forcing the \textsf{KeyGen}() algorithm until it obtains the required
signing key. As a standard, cryptographic literature only considers
\emph{probabilistic polynomial-time} (PPT) adversaries --- polynomial in the
security parameter $\lambda$. Not considering quantum computers, the strongest
practical computers to date can be approximated by PPT, so they encompass all
relevant real-world attack scenarios. The aforementioned brute-force attack is
therefore exceedingly unlikely to succeed for large enough key spaces ---
typically of exponential size in $\lambda$.

Unfortunately, a computational treatment of digital signatures security is at
odds with formal verification. In the latter, we would like to categorically
rule out the exponentially small probability of a successful forgery in a
principled manner. We achieve this by replacing the construction with an
\emph{idealized} digital signatures functionality which never permits forgeries
(not even with \emph{negligible} probability), as defined
in~\cite{DBLP:conf/csfw/Canetti04}. At a high level, this
functionality plays the role of a single ``trusted signatures server'' that is
common for all parties. Parties request the signing and verification of
messages and the functionality responds accordingly, storing the message-party
pair on every signature request and responding whether the given message-party
pair has been stored on every verification request. Crucially, the
functionality is incorruptible, making forgeries impossible. This approach
bridges the sensibilities of real-world cryptography with the requirements of
formal verification.

A salient question is: why is the replacement of the construction with the
functionality valid? The answer comes from the \emph{simulation-based
cryptographic paradigm}. This paradigm employs an \emph{indistinguishability
argument}, according to which \emph{every} external PPT observer (commonly
called \emph{environment}) is unable to distinguish between interactions with
the construction versus the functionality, except with negligible probability,
thus justifying our use of the ideal functionality.

Given our use of a forgery-free signatures functionality, a second model
complication can be simplified: the PPT limitation on the adversary can be
dropped, allowing for any, even unbounded, adversaries. This enables modelling
the adversary in Why3 using the \texttt{any} keyword. Statically quantifying
over all PPT machines has historically proven exceedingly
difficult~\cite{DBLP:conf/pldi/LiaoHM19}, therefore avoiding the need for a PPT
bound is highly desirable.

